Active Learning for Text-to-Speech Synthesis with Informative Sample Collection

The construction of high-quality datasets is a cornerstone of modern text-to-speech (TTS) systems. However, the increasing scale of available data poses significant challenges, including storage constraints. To address these issues, we propose a TTS corpus construction method based on active learning. Unlike traditional feed-forward and model-agnostic corpus construction approaches, our method iteratively alternates between data collection and model training, thereby focusing on acquiring data that is more informative for model improvement. This approach enables the construction of a data-efficient corpus. Experimental results demonstrate that the corpus constructed using our method enables higher-quality speech synthesis than corpora of the same size.

==> chapter6/apsipa/single_table.tex <==
\multirow{1}{*}{$58500$}
  &Unselected & $1157 / 2719 (42.6\%)$ & $1157 / 2719 (42.6\%)$ & -\\ \midrule
\multirow{1}{*}{$2454$}
  &Initial corpus & $1673 / 2719 (61.5\%)$ & $87 / 105 (82.9\%)$ & $1586 / 2614 (60.7\%)$\\ \midrule
\multirow{2}{*}{$3943$}
  &Baseline & $1810 / 2719 (66.6\%)$ & $\mathbf{467 / 480 (97.3\%)}$ & $1343 / 2239 (60.0\%)$\\
  &Ours & $\mathbf{1930 / 2719 (71.0\%)}$ & $147 / 281 (52.3\%)$ & $\mathbf{1783 / 2438 (73.1\%)}$


==> chapter6/python/single_table.tex <==
\multirow{1}{*}{$58500$}
  &Unselected & $1157 / 2719 (42.6\%)$ & $1157 / 2719 (42.6\%)$ & -\\ \midrule
\multirow{1}{*}{$2454$}
  &Initial corpus & $1673 / 2719 (61.5\%)$ & $87 / 105 (82.9\%)$ & $1586 / 2614 (60.7\%)$\\ \midrule
\multirow{2}{*}{$3943$}
  &Ours-Single & $\mathbf{1930 / 2719 (71.0\%)}$ & $147 / 281 (52.3\%)$ & $\mathbf{1783 / 2438 (73.1\%)}$\\
  &Baseline (3943) & $1810 / 2719 (66.6\%)$ & $\mathbf{467 / 480 (97.3\%)}$ & $1343 / 2239 (60.0\%)$

